An Efficient Low-Complexity RSMA Scheme for Multi-User Decode-and-Forward Relay Systems

Rate-Splitting Multiple Access (RSMA) is a promising strategy for ensuring robust transmission in multi-antenna wireless systems. In this paper, we investigate the performance of RSMA in a downlink Decode-and-Forward (DF) relay scenario under two phases with imperfect Channel State Information (CSI) at the transmitter and the relay. In particular, in the first phase, the Base Station (BS) initially transmits to both BS Users (BUs) and the relay. In the second phase, the relay decodes and forwards the received signals to Relay Users (RUs) outside the BS coverage area. Furthermore, we investigate a scenario where the relay broadcasts a common stream intended for the RUs in the second phase. Due to the broadcast nature of the transmission, this stream is inadvertently received by both the RUs and the BUs. Concurrently, the BS utilizes Spatial Division Multiple Access (SDMA) to transmit private streams to the BUs, resulting in BUs experiencing residual interference from the common stream transmitted from relay. Incorporating this residual common stream interference into our model results in a significant enhancement of the overall sum-rate achieved at the BUs. We derive a tractable lower bound on the ergodic sum-rates, enables us to develop closed-form solutions for power allocation that maximize the overall sum-rate in both phases. Extensive simulations validate that our proposed power allocation algorithm, in conjunction with a low-complexity precoder, significantly improves the sum-rate performance of DF relay RSMA networks compared to the SDMA-based benchmark designs under imperfect CSI at the transmitter and relay.

==> AcronymList.tex <==
\usepackage{etoolbox}
\makeatletter
\newif\ifAC@uppercase@first%
\def\Aclp#1{\AC@uppercase@firsttrue\aclp{#1}\AC@uppercase@firstfalse}%
\def\AC@aclp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acl{#1}s%
	\fi%
}%
\def\Acp#1{\AC@uppercase@firsttrue\acp{#1}\AC@uppercase@firstfalse}%
\def\AC@acp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@ac{#1}s%
	\fi%
}%
\def\Acfp#1{\AC@uppercase@firsttrue\acfp{#1}\AC@uppercase@firstfalse}%
\def\AC@acfp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acf{#1}s%
	\fi%
}%
\def\Acsp#1{\AC@uppercase@firsttrue\acsp{#1}\AC@uppercase@firstfalse}%
\def\AC@acsp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acs{#1}s%
	\fi%
}%
\edef\AC@uppercase@write{\string\ifAC@uppercase@first\string\expandafter\string\MakeUppercase\string\fi\space}%
\def\AC@acrodef#1[#2]#3{%
	\@bsphack%
	\protected@write\@auxout{}{%
		\string\newacro{#1}[#2]{\AC@uppercase@write #3}%
	}\@esphack%
}%
\def\Acl#1{\AC@uppercase@firsttrue\acl{#1}\AC@uppercase@firstfalse}
\def\Acf#1{\AC@uppercase@firsttrue\acf{#1}\AC@uppercase@firstfalse}
\def\Ac#1{\AC@uppercase@firsttrue\ac{#1}\AC@uppercase@firstfalse}
\def\Acs#1{\AC@uppercase@firsttrue\acs{#1}\AC@uppercase@firstfalse}
\robustify\Aclp
\robustify\Acfp
\robustify\Acp
\robustify\Acsp
\robustify\Acl
\robustify\Acf
\robustify\Ac
\robustify\Acs
\makeatother

\acrodef{AWGN}[AWGN]{Additive White Gaussian Noise}
\acrodef{SE}[SE]{Spectral Efficiency}
\acrodef{CM}[CM]{Constant Modulus}
\acrodef{BS}[BS]{Base Station}
\acrodef{AO}[AO]{Alternating Optimization}
\acrodef{mmWave}[mmWave]{millimeter-Wave}
\acrodef{MU-MIMO}[MU-MIMO]{Multi-User Multiple-Input Multiple-Output}
\acrodef{MU-MISO}[MU-MISO]{Multi-User Multiple-Input Single-Output}
\acrodef{AF}[AF]{Amplify-and-Forward}
\acrodef{DF}[DF]{Decode-and-Forward}
\acrodef{RF}[RF]{radio frequency}
\acrodef{BB}[BB]{baseband}
\acrodef{iid}[i.i.d.]{independently and identically distributed}

\acrodef{RS}[RS]{Rate Splitting}
\acrodef{MIMO}[MIMO]{Multiple-Input Multiple-Output}
\acrodef{MISO}[MISO]{Multiple-Input Single-Output}
\acrodef{DL}[DL]{Downlink}
\acrodef{ZF}[ZF]{Zero-Forcing}
\acrodef{SVD}[SVD]{Singular Value
Decomposition}
\acrodef{RSMA}[RSMA]{Rate-Splitting Multiple Access}
\acrodef{6G}[6G]{sixth-generation}
\acrodef{subTHz}[sub-THz]{sub-Terahertz}
\acrodef{THz}[THz]{Terahertz}
\acrodef{OMA}[OMA]{Orthogonal Multiple Access}
\acrodef{MUI}[MUI]{Multi-User Interference}
\acrodef{MRT}[MRT]{Maximum Ratio Transmission}
\acrodef{DoF}[DoF]{Degrees of Freedom}
\acrodef{SINR}[SINR]{
Signal-to-Interference-plus-Noise Ratio}
\acrodef{SDMA}[SDMA]{
Space-Division Multiple Access}
\acrodef{CSIT}[CSIT]{Channel State Information at the Transmitter}
\acrodef{CSIR}[CSIR]{CSI at the Receiver}
\acrodef{SIC}[SIC]{Successive Interference Cancellation}
\acrodef{NDF}[NDF]{Non-regenerative DF}
\acrodef{AER}[AER]{Approximated Ergodic Rates}
\acrodef{SU}[SU]{Single-User}
\acrodef{MU}[MU]{Multi-User}
\acrodef{CDRT}[CDRT]{Coordinated Direct and Relay Transmission}
\acrodef{NOMA}[NOMA]{Non-Orthogonal Multiple Access}
\acrodef{CRS}[CRS]{Cooperative RS}
\acrodef{CSI}[CSI]{Channel State Information}
\acrodef{URLLC}[URLLC]{Ultra Reliable Low Latency Communications}
\acrodef{SNR}[SNR]{Signal-to-Noise Ratio}
\acrodef{BC}[BC]{Broadcast}
\acrodef{LOS}[LoS]{Line-of-Sight}
\acrodef{ESR}[ESR]{Ergodic Sum Rate}
\acrodef{AESR}[AESR]{Approximated ESR}
\acrodef{AER}[AER]{Approximated ER}
\acrodef{PCI}[PCI]{Partially Common Interference}
\acrodef{FCI}[FCI]{Fully Common Interference}
\acrodef{BU}[BU]{BS User}
\acrodef{RU}[RU]{Relay User}
\acrodef{CSCG}[CSCG]{Circularly Symmetric Complex Gaussian}
\acrodef{NLOS}[NLoS]{Non-LoS}
\acrodef{ER}[ER]{Ergodic Rate}
\acrodef{GMI}[GMI]{Generalized Mutual Information}
\acrodef{}[]{}
\acrodef{}[]{}

